Real-Time Model Checking Support for AADL

We describe a model-checking toolchain for the behavioral verification of AADL models that takes into account the realtime semantics of the language and that is compatible with the AADL Behavioral Annex. We give a high-level view of the tools and transformations involved in the verification process and focus on the support offered by our framework for checking user-defined properties. We also describe the experimental results obtained on a significant avionic demonstrator, that models a network protocol in charge of data communications between an airplane and ground stations.

==> biblio.tex <==
\bibitem{ADELE} ADELE: a versatile system architecture graphical
  editor based on AADL.\newblock
  \url{http://gforge.enseeiht.fr/projects/adele/}

\bibitem{SAE} SAE Aerospace.  Architecture Analysis \& Design Language
  (AADL).\newblock AS-5506, SAE International, 2004.

\bibitem{ARINC} Airlines electronic engineering committee. \newblock
  {Avionics Application Software Standard Interface, {ARINC}
    Specification 653}. \newblock 1997.

\bibitem{bipaadl16} A. Basu, M. Bozga, and J. Sifakis.\newblock
  Modeling heterogeneous real-time systems in BIP.\newblock In
  \emph{Proc. of SEFM -- IEEE Software Engineering and Formal
    Methods}, 2006.

% \bibitem{bipaadl4} M. Chkouri, A. Robert, M. Bozga,
%   J. Sifakis.\newblock Translating AADL into BIP -- application to the
%   verification of real-time systems.\newblock In \emph{Proc. of MoDELS
%     ACES-MB -- Model Based Architecting and Construction of Embedded
%     Systems}, 2008.

\bibitem{mam2} R. B. Franca, J.-P. Bodeveix, D. Chemouil, M. Filali,
  D. Thomas, J.-F. Rolland.  \newblock The AADL behaviour annex,
  experiments and roadmap.\newblock In \emph{Proc. of ICECCS -- IEEE
    International Conference on Engineering of Complex Computer
    Systems}, 2007.

% \bibitem{model3} P.-A. Muller, F. Fleurey, D. Vojtisek, Zo\'{e} Drey,
%   Damien Pollet, F. Fondement, P. Studer, and J.-M. J\'{e}z\'{e}uel.
%   \newblock On executable meta-languages applied to model
%   transformations.\newblock In \emph{Proc. of MoDELS -- Model
%     Transformations In Practice}, 2005.

% \bibitem{Hal07} E. Jahier, N. Halbwachs, P. Raymond, X. Nicollin,
%   D. Lesens. \newblock Virtual Execution of AADL Models via a
%   Translation into Synchronous Programs. \newblock In \emph{Proc. of
%     EMSOFT -- ACM \& IEEE international conference on Embedded
%     software}, 2007.

% \bibitem{model4} F. Jouault, and I. Kurtev.\newblock Transforming
%   Models with ATL.\newblock In \emph{Proc. of MoDELS -- Model
%     Transformations in Practice}, 2005.

% \bibitem{OAW} OAW, \url{http://www.openarchitectureware.org/}.

% \bibitem{OCL} OCL, UML 2.0 Object Constraint Language.

\bibitem{tpn} P. M. Merlin and D. J. Farber.\newblock Recoverability
  of communication protocols: Implications of a theoretical
  study.\newblock \emph{IIEEE Transactions on Computers},
  24(9):1036--1043, 1976.

\bibitem{tina8} B. Berthomieu, P.-O. Ribet, and F. Vernadat.\newblock
  The tool TINA -- Construction of Abstract State Spaces for Petri
  Nets and Time Petri Nets.\newblock \emph{International Journal of
    Production Research}, 42(14), 2004.

% \bibitem{cadp9} H. Garavel, F. Lang, R. Mateescu, W. Serve.\newblock
%   CADP: A Toolbox for the Construction and Analysis of Distributed
%   Processes.\newblock In \emph{Proc. of CAV -- Int. Conf. On Computer
%     Aided Verification}, 2007.  

\bibitem{fiacre10} B. Berthomieu, J. P. Bodeveix, M. Filali,
  H. Garavel, F. Lang, F. Peres, R. Saad, J. Stoecker,
  F. Vernadat.\newblock The syntax and semantics of Fiacre.\newblock
  Research Report LAAS 07264, 2007.

% \bibitem{bipaadlPi} L. Pi, J.-P. Bodeveix, M. Filali.\newblock
%   Modeling AADL Data Communication with BIP.\newblock Preprint, 2009.

% \bibitem{selt} S.  Chaki, E.  M. Clarke, J. Ouaknine, N. Sharygina, N.
%   Sinha.\newblock State/Event-based Software Model Checking.\newblock
%   In \emph{Proc. of IFM -- Integrated Formal Methods}, LNCS Vol. 2999,
%   2004.

% \bibitem{aadltla5} J.-F. Rolland, J.-P. Bodeveix, D. Chemouil,
%   M. Filali, D. Thomas.\newblock Towards a formal semantics for AADL
%   execution model.\newblock In \emph{Proc. of ERTS -- European
%     Congress on Embedded Real-Time Software}, 2008.

% \bibitem{modes14} J.-F. Rolland, J.-P. Bodeveix, M. Filali, D. Thomas,
% D. Chemouil.\newblock Modes in asynchronous systems.\newblock In
% \emph{Proc. of UML\&AADL}, 2008.

\bibitem{topcased11} Topcased: "Toolkit in OPen-source for Critical
  Apllications and SystEms Development",
  \url{http://www.topcased.org}.  

% \bibitem{BB15} B. Berthomieu, and F. Vernadat.\newblock State Space
%   Abstractions for Time Petri Nets.\newblock Handbook of Real-Time and
%   Embedded Systems, Chapman \& Hall, 2007.  

% \bibitem{cotre20} J.-M. Farines, B. Berthomieu, J.-P. Bodeveix,
%   P. Dissaux, P. Farail, M. Filali, P. Gaufillet, H. Hafidi,
%   J.-L. Lambert, P. Michel, and F. Vernadat.  \newblock The Cotre
%   Project: Rigorous Software Development for Real Time Systems in
%   Avionics. \newblock In \emph{Proc. of FMICS -- Formal Methods for
%     Industrial Critical Systems}, vol. 80 of ENTCS, 2003.

% \bibitem{aadluml6} C. Andr\'{e}, F. Mallet, R. de Simone.\newblock Modeling of
%   immediate vs. delayed data communications: from AADL to UML
%   Marte.\newblock In \emph{Forum on specification \& Design Languages},
%   2007.

% \bibitem{feileraadl7} P. Feiler.\newblock Efficient embedded runtime
%   systems through port communication optimization.\newblock in
%   \emph{Proc. of ICECCS -- IEEE International Conference on
%     Engineering of Complex Computer Systems}, 2008.

% \bibitem{ver06} T. Vergnaud.\newblock Mod\'{e}lisation des
%   syst\`{e}mes temps-r\'{e}el r\'{e}partis embarqu\'{e}s pour la
%   g\'{e}n\'{e}ration automatique d'applications formellement
%   v\'{e}rifi\'{e}es.\newblock PhD Thesis, \'{E}cole nationale
%   sup\'{e}rieure des t\'{e}l\'{e}communications, 2006.

\bibitem{osate21} The SEI AADL Team.\newblock \emph{An Extensible Open
    Source AADL Tool Environment (OSATE)}.\newblock Software
  Engineering Institute, 2006.

\bibitem{aadl09} B. Berthomieu, J.-P. Bodeveix, C. Chaudet, S. Dal
  Zilio, M. Filali, F. Vernadat.\newblock Formal Verification of AADL
  Specifications in the Topcased Environment.\newblock In
  \emph{Proc. of Ada Europe 2009 -- 14th Ada-Europe International
    Conference}, LNCS Vol. 5570, 2009.

% %%% Local Variables: 
% %%% mode: latex
% %%% TeX-master: "aadltina"
% %%% End: 


